Energy-Efficient Computation with DVFS using Deep Reinforcement Learning for Multi-Task Systems in Edge Computing

Finding an optimal energy-efficient policy that is adaptable to underlying edge devices while meeting deadlines for tasks has always been challenging. This research studies generalized systems with multi-task, multi-deadline scenarios with reinforcement learning-based DVFS for energy saving for periodic soft real-time applications on edge devices. This work addresses the limitation of previous work that models a periodic system as a single task and single-deadline scenario, which is too simplified to cope with complex situations. The method encodes time series data in the Linux kernel into information that is easy to interpret for reinforcement learning, allowing the system to generate DVFS policies to adapt system patterns based on the general workload. For encoding, we present two different methods for comparison. Both methods use only one performance counter: system utilization, and the kernel only needs minimal information from the userspace. Our method is implemented on Jetson Nano Board (2GB) and is tested with three fixed multitask workloads, which are three, five, and eight tasks in the workload, respectively. For randomness and generalization, we also designed a random workload generator to build different multitask workloads to test. Based on the test results, our method could save 3%-10% power compared to Linux built-in governors.

==> Sections/introduction.tex <==
\section{Introduction}

%\subsection{The Limitation of Single Task Single Deadline System}
\subsection{System Model Context}
Soft real-time systems are often used for processing periodic tasks that are time-constrained but  not strictly, and they have many applications. Here are some examples: optimized control
software for automobiles ~\cite{minaeva2020control} involving periodical sensing, computing,
and driving tasks that have real-time
requirements; a
smart-farm system where most communication is periodic~\cite{nobrega2019iot}; and a system that periodically monitors of soil health~\cite{ramson2021self}.
%\cite{nobrega2019iot} proposed an architecture for smart farms where most communication is periodic. \cite{ramson2021self} constructed a real-time system for periodic monitoring of soil health.

For these systems, performance and energy are two indicators that interest researchers. A previous work \cite{zhou2023cpu} modelled them as a single task with a single deadline system and proposed a model-free method to save energy for the system while ensuring performance. However, this modelling method has its limitations because of oversimplification. In real-world applications, there is usually more than one task in one period. Some of these tasks could contain dependencies that need to be executed sequentially, such as getting and processing data \cite{lee2022probabilistically} \cite{teslyuk2020optimal} \cite{manogaran2020isof}. Some tasks can be executed in parallel, such as the system using multiple sensors which can acquire data simultaneously \cite{salman2021systematic} \cite{liu2020continuous} \cite{yuan2021design}. 

The previous work \cite{zhou2023cpu} could not adequately model the complex situation with only a single task and a single deadline. In this work, we study systems that have multiple tasks in one period, and each of these tasks has its deadlines. 
%In this situation, we further modified our original method to suit the multitasking situation.

\subsection{Problem Statement and Proposed Method}
%We treat the tasks that the system runs in one period as a task set. 
We consider multi-tasks in a task set that runs periodically. 
Each task $task_{i}$ has its timestamp of start $start_i$, execution time $exet_{i}$, timestamp of finish $finish_{i}$ and deadline $ddl_{i}$. For simplicity, we assume each task is independent of the other and their startup depends only on the predefined setting time. During each period, the task set is executed once for a total deadline time of $T$, which is the deadline for the last task. Others' deadlines cannot exceed $T$.


\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth]{Figure/definition.png}
  \caption{Deadline Missing Example: A Multi-Task set with Multi-Deadline on Multi-Core
  %System definition and method to solve.
  }
  \label{fig:definition}
\end{figure*}


Fig.~\ref{fig:definition} gives a detailed example of the type of systems studied in this paper. In this example, a real-time task set consists of five tasks that run on a device with four cores. \textcolor{black}{This series of tasks runs periodically on the system. Our aim is to find a adaptable policy that can save as much system energy as possible without causing tasks to miss their deadlines  on the multi-core system. The only reason a deadline is missing on a single-tasking system is that the system dose not run with a high enough frequency.
%Exceeding the deadline on a single-tasking system can only be due to one reason: the system does not run with a high enough frequency. 
However, various situations may cause a timeout during a run on multicore systems, as shown in Fig.~\ref{fig:definition}.  On a multi-core system, a task may miss the deadline because appropriate frequencies are not used, the same as on single-tasking systems. A previous task on the same core or tasks on other cores that have migrated to this core may also cause the deadline to be missed.}
\textcolor{black}{Thus, in a multi-task system, the causes for task timeouts become much more complex. How can the frequencies be managed without causing tasks to miss their deadlines and save as much energy as possible? Possible solutions are constructing offline mathematical models \cite{chang2020real} \cite{xu2024energy} \cite{wu2023energy} \cite{houssam2020hpc} \cite{chen2020scheduling} or solving the problem automatically with machine learning-based methods \cite{hoffmann2021online} \cite{zhan2019power} \cite{li2024deep} \cite{chen2021energy} \cite{fettes2018dynamic}. \cite{panda2022energy} \cite{zhou2021deadline} \cite{zhou2023cpu}}  
% \textcolor{black}{add references}


\textcolor{black}{To solve this problem, we propose to combine Reinforcement Learning (RL) and Dynamic Voltage and Frequency Scaling (DVFS) with an encoding of system state to capture the deadline of multi-tasks and multi-core system status and make predictions.} DVFS is an energy-saving method which adapts voltage and frequency dynamically to satisfy the system's needs. Linux has some built-in DVFS governors \cite{zhou2023profiling}, such as \textit{Ondemand} and \textit{Conservative}. They make predictions based on the utilization in the previous period, that is, they assume the next period is the same as the previous one. Also, they adjust the frequency based on the max load of the system. Our method uses Double Deep Q Learning (DDQN) \cite{van2016deep} to train a DVFS policy since every execution of the task set which reaches $T$ time could be seen as an episode. This task set will be executed each period which indicates that the events that happened in each period are almost the same. The governor could predict the events and system states once a good policy is driven.

\subsection{Method Overview}
An overview of our method is shown in Fig.~\ref{fig:overview}. In the Linux kernel, we insert an encoder and neural network. The encoder is responsible for encoding the system information from the last period and the observations from this period. The encoded data will be sent to networks with frequency as action to calculate the corresponding Q value. Based on the max Q value, the governor chooses the corresponding frequency for the next period. If training is required, all the data will be recorded and sent to userspace to update the networks. The new network will be sent to the kernel for testing. After around 400 trainings, the governor could get a good policy. 

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{Figure/overview.png}
  \caption{An overview of our proposed method.}
  \label{fig:overview}
\end{figure}

Our proposed method is more accurate than traditional Linux built-in governors based on the following reasons. Our method uses the temporal series information in the kernel including average and max utilization. While the Linux built-in governors only use max load from the last period which means they have little information and do not have an overall judgement of the workload and system status.

Compared with the previous method for a single task and single deadline situation \cite{zhou2023cpu}, our new method is not a pure model-free strategy as the task number needs to be passed to the kernel. Besides this information, the method could encode the system parameters to useful information which be learnt by RL. We are the first to propose a method that is applied to multitasking with multiple deadlines in a soft real-time system which can save 3\% - 10\% power compared with Linux built-in governor. 
